Matryoshka: Fuzzing Deeply Nested Branches

Greybox fuzzing has made impressive progress in recent years, evolving from heuristics-based random mutation to approaches for solving individual path constraints. However, they have difficulty solving path constraints that involve deeply nested conditional statements, which are common in image and video decoders, network packet analyzers, and checksum tools. We propose an approach for addressing this problem. First, we identify all the control flow-dependent conditional statements of the target conditional statement. Next, we select the data flow-dependent conditional statements. Finally, we use three strategies to find an input that satisfies all conditional statements simultaneously. We implemented this approach in a tool called Matryoshka and compared its effectiveness on 13 open source programs against other state-of-the-art fuzzers. Matryoshka found significantly more unique crashes than AFL, QSYM, and Angora. We manually classified those crashes into 41 unique new bugs, and obtained 12 CVEs. Our evaluation also uncovered the key technique contributing to Matryoshka's impressive performance: it collects only the nesting constraints that may cause the target conditional statements unreachable, which greatly simplifies the constraints that it has to solve.

==> Makefile <==
# You may override this variable from the command line. E.g.:
# make target=foo
# make clean target=foo
target = main
papersize = letter

.PHONY : clean all

all : $(patsubst %,%.pdf,$(target))

clean :
	for i in aux log bbl blg bcf out run.xml pdf; do \
		rm -f $(patsubst %,%.$$i,$(target)); \
	done
	-rm -f *~

# You may append other dependencies
%.pdf : %.tex %.bib
	# dot -Tpdf post-dom.dot -o ./figure/post_dom.pdf
	$(eval basename = $(patsubst %.tex,%,$<))
	xelatex -papersize=$(papersize) $(basename)
	biber $(basename)
	xelatex -papersize=$(papersize) $(basename)
	xelatex -papersize=$(papersize) $(basename)

